Circumstellar molecular composition of the oxygen-rich AGB star IK~Tau: II. In-depth non-LTE chemical abundance analysis

Aims: Little information exists on the circumstellar molecular abundance stratifications of many molecules. The aim is to study the circumstellar chemical abundance pattern of 11 molecules and isotopologs ($^{12}$CO, $^{13}$CO, SiS, $^{28}$SiO, $^{29}$SiO, $^{30}$SiO, HCN, CN, CS, SO, SO$_2$) in the oxygen-rich evolved star IK~Tau. Methods: We have performed an in-depth analysis of a large number of molecular emission lines excited in the circumstellar envelope around IK~Tau. The analysis is done based on a non-local thermodynamic equilibrium (non-LTE) radiative transfer analysis, which calculates the temperature and velocity structure in a self-consistent way. The chemical abundance pattern is coupled to theoretical outer wind model predictions including photodestruction and cosmic ray ionization. Not only the integrated line intensities, but also the line shapes, are used as diagnostic tool to study the envelope structure. Results: The deduced wind acceleration is much slower than predicted from classical theories. SiO and SiS are depleted in the envelope, possibly due to the adsorption onto dust grains. For HCN and CS a clear difference with respect to inner wind non-equilibrium predictions is found, either indicating uncertainties in the inner wind theoretical modeling or the possibility that HCN and CS (or the radical CN) participate in the dust formation. The low signal-to-noise profiles of SO and CN prohibit an accurate abundance determination; the modeling of high-excitation SO$_2$ lines is cumbersome, possibly related to line misidentifications or problems with the collisional rates. The SiO isotopic ratios ($^{29}$SiO/$^{28}$SiO and $^{30}$SiO/$^{28}$SiO) point toward an enhancement in $^{28}$SiO compared to results of classical stellar evolution codes. Predictions for H$_2$O lines in the spectral range of the Herschel/HIFI mission are performed. [abbreviated]

==> out <==
This is pdfTeXk, Version 3.1415926-1.40.9 (Web2C 7.5.7)
 %&-line parsing enabled.
entering extended mode
(./decinl.tex
LaTeX2e <2005/12/01>
Babel <v3.8l> and hyphenation patterns for english, usenglishmax, dumylang, noh
yphenation, german-x-2008-06-18, ngerman-x-2008-06-18, ancientgreek, ibycus, ar
abic, basque, bulgarian, catalan, pinyin, coptic, croatian, czech, danish, dutc
h, esperanto, estonian, farsi, finnish, french, galician, german, ngerman, mono
greek, greek, hungarian, icelandic, indonesian, interlingua, irish, italian, la
tin, mongolian, mongolian2a, bokmal, nynorsk, polish, portuguese, romanian, rus
sian, sanskrit, serbian, slovak, slovenian, spanish, swedish, turkish, ukenglis
h, ukrainian, uppersorbian, welsh, loaded.
(./aa.cls
Document Class: aa 2010/20/02 v7.0 
LaTeX document class for Astronomy and Astrophysics journal
(/usr/share/texmf/tex/latex/base/fleqn.clo)) (./natbib.sty)
(/usr/share/texmf/tex/latex/tools/afterpage.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/lib/texmf/tex/latex/config/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/lib/texmf/tex/latex/config/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/psnfss/times.sty)
(/usr/share/texmf/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texmf/tex/latex/subfigure/subfigure.cfg))
(/usr/share/texmf/tex/generic/babel/babel.sty
(/usr/share/texmf/tex/generic/babel/english.ldf
(/usr/share/texmf/tex/generic/babel/babel.def))) (./decinl.aux)
(/usr/share/texmf/tex/latex/psnfss/ot1ptm.fd)
(/usr/share/texmf/tex/latex/psnfss/omsptm.fd)
(/usr/share/texmf/tex/latex/psnfss/ot1phv.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
Underfull \hbox (badness 1168) in paragraph at lines 92--92
 \OT1/phv/m/sl/9 Aims. \OT1/ptm/m/n/9 Little ob-ser-va-tional in-for-ma-tion ex
-ists on the cir-cum-stel-lar molec-u-lar abun-dance strat-i-fi-ca-tions of man
y molecules. 

Underfull \hbox (badness 10000) in paragraph at lines 92--92
[][] \OT1/ptm/m/it/9 Send off-print re-quests to\OT1/ptm/m/n/9 : L. Decin, e-ma
il:
[1]
Underfull \vbox (badness 6396) has occurred while \output is active [2]
Overfull \hbox (5.88487pt too wide) in paragraph at lines 200--284
[][] 

Underfull \hbox (badness 1377) in paragraph at lines 284--284
\OT1/ptm/m/n/9 (3) Sch[]oier et al. (2007b); (4) Gonz[]alez Delgado et al. (200
3);

Underfull \hbox (badness 10000) in paragraph at lines 284--286


LaTeX Warning: Float too large for page by 29.39026pt on input line 286.


Underfull \vbox (badness 10000) has occurred while \output is active [3]
<drawing_agb4.ps>
Underfull \vbox (badness 10000) has occurred while \output is active [4]
<Cherchneff_Willacy.ps>
Overfull \hbox (6.0pt too wide) in paragraph at lines 451--463
 [] 
[5]
Underfull \hbox (badness 1163) in paragraph at lines 496--507
\OT1/ptm/m/n/10 tem-per-a-ture, ve-loc-ity and den-sity struc-ture, are de-ter-
mined

Underfull \vbox (badness 10000) has occurred while \output is active [6]
Overfull \hbox (3.70998pt too wide) in paragraph at lines 523--541
[][] 
[7] <velocity.ps> <structure_IKTau_Karen_new4.ps> <willacy_observed_new1.ps>
<willacy_observed_new2.ps>
Underfull \hbox (badness 10000) in paragraph at lines 737--737

<CO_results_mlineCO_MARCS.ps> [8]
Underfull \hbox (badness 2293) in paragraph at lines 755--756
\OT1/ptm/m/n/10 abun-dance as-sumed in all ob-ser-va-tional stud-ies (see also
[9] <HCN3-2_IRAM.ps> <HCN4-3_APEX.ps> [10]
Underfull \vbox (badness 10000) has occurred while \output is active
Underfull \vbox (badness 10000) has occurred while \output is active [11]
<SiS5-4_OSO.ps> <SiS6-5_OSO.ps> <SiS8-7_IRAM.ps> <SiS12-11_IRAM.ps>
<SiS12-11_JCMT.ps> <SiS16-15_APEX.ps> <SiS17-16_APEX.ps> <SiS19-18_JCMT.ps>
<SiS19-18_APEX.ps> <SiS20-19_APEX.ps>
Underfull \vbox (badness 10000) has occurred while \output is active [12]
<28SiO7-6_APEX.ps> <28SiO8-7_APEX.ps> <SiO_GonzalesDelgado2.ps>
<SiO_pred_Gonzales.ps> <29SiO7-6_APEX.ps> <29SiO8-7_APEX.ps>
<30SiO7-6_APEX.ps> <30SiO8-7_APEX.ps> [13]
Underfull \hbox (badness 10000) in paragraph at lines 923--924
[]\OT1/ptm/m/n/10 The de-rived iso-topic ra-tios in the en-ve-lope are
<CS6-5_APEX.ps> <CS7-6_APEX.ps> [14] <CN3034-2023_APEX.ps>
<CN3045-2034_APEX.ps> <SO7-6_APEX.ps> <SO8-7_APEX.ps> [15]
<SO2_14311-14212_IRAM.ps> <SO2_431-422_IRAM.ps> <SO2_331-322_IRAM.ps>
<SO2_533-524_IRAM.ps> <SO2_331-220_APEX.ps> <SO2_17117-16016_APEX.ps>
<SO2_431-322_APEX.ps> <SO2_13212-12111_APEX.ps> <SO2_533-422_APEX.ps>
<SO2_14410-14311_APEX.ps> [16]
Underfull \vbox (badness 2970) has occurred while \output is active [17]
Overfull \hbox (4.74026pt too wide) in alignment at lines 1143--1146
[][][] []
<H2O_profiles_newb.ps>
Underfull \hbox (badness 1490) in paragraph at lines 1181--1181
[]\OT1/ptm/b/n/9 Table 8. |\OT1/ptm/m/n/9 Line fre-quen-cies, up-per en-ergy le
v-els and Einstein A-

Overfull \hbox (8.63934pt too wide) in paragraph at lines 1184--1205
 [] 
[18] <H2O_profiles_nub.ps>
Overfull \hbox (6.0pt too wide) in paragraph at lines 1224--1225
[][] 
[19] <H2O_profiles_paramb.ps>
Overfull \hbox (6.0pt too wide) in paragraph at lines 1241--1242
[][] 
<compare_BB_MARCS.ps>
Overfull \hbox (6.0pt too wide) in paragraph at lines 1247--1248
[][] 
[20] <EinsteinCO.ps>
Underfull \hbox (badness 3482) in paragraph at lines 1299--1299
[]\OT1/ptm/b/n/9 FigureA.1. |\OT1/ptm/m/n/9 Comparison be-tween the tran-si-tio
n fre-quen-cies and
<EinsteinSiO.ps>
Underfull \hbox (badness 3482) in paragraph at lines 1326--1326
[]\OT1/ptm/b/n/9 FigureA.2. |\OT1/ptm/m/n/9 Comparison be-tween the tran-si-tio
n fre-quen-cies and

Underfull \hbox (badness 1803) in paragraph at lines 1333--1351
\OT1/ptm/m/n/10 for Molecular Spectroscopy (CDMS, M[]uller et al. 2005).
[21] <EinsteinSiS.ps>
Underfull \hbox (badness 3482) in paragraph at lines 1357--1357
[]\OT1/ptm/b/n/9 FigureA.3. |\OT1/ptm/m/n/9 Comparison be-tween the tran-si-tio
n fre-quen-cies and
<EinsteinH2O.ps>
Underfull \hbox (badness 3482) in paragraph at lines 1453--1453
[]\OT1/ptm/b/n/9 FigureA.4. |\OT1/ptm/m/n/9 Comparison be-tween the tran-si-tio
n fre-quen-cies and
[22] (./decinl.bbl
Underfull \vbox (badness 10000) has occurred while \output is active [23])
[24] (./decinl.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information)
Output written on decinl.dvi (24 pages, 194636 bytes).
Transcript written on decinl.log.

